Resolving the Dust-to-Metals Ratio and CO-to-H$_2$ Conversion Factor in the Nearby Universe

We investigate the relationship between the dust-to-metals ratio (D/M) and the local interstellar medium environment at ~2 kpc resolution in five nearby galaxies: IC342, M31, M33, M101, and NGC628. A modified blackbody model with a broken power-law emissivity is used to model the dust emission from 100 to 500 um observed by Herschel. We utilize the metallicity gradient derived from auroral line measurements in HII regions whenever possible. Both archival and new CO rotational line and HI 21 cm maps are adopted to calculate gas surface density, including new wide field CO and HI maps for IC342 from IRAM and the VLA, respectively. We experiment with several prescriptions of CO-to-H$_2$ conversion factor, and compare the resulting D/M-metallicity and D/M-density correlations, both of which are expected to be non-negative from depletion studies. The D/M is sensitive to the choice of the conversion factor. The conversion factor prescriptions based on metallicity only yield too much molecular gas in the center of IC342 to obtain the expected correlations. Among the prescriptions tested, the one that yields the expected correlations depends on both metallicity and surface density. The 1-$\sigma$ range of the derived D/M spans 0.40-0.58. Compared to chemical evolution models, our measurements suggest that the dust growth time scale is much shorter than the dust destruction time scale. The measured D/M is consistent with D/M in galaxy-integrated studies derived from infrared dust emission. Meanwhile, the measured D/M is systematically higher than the D/M derived from absorption, which likely indicates a systematic offset between the two methods.

==> tab_IC342VLA.tex <==
\begin{deluxetable*}{cccccccc}
\tablecaption{Summary of \HI\ observation blocks of IC342.\label{tab: hi_blocks}}
\tablecolumns{11}
\tablewidth{0pt}
\tablehead{
\colhead{Project Code} &
\colhead{Date\tablenotemark{a}}          & \colhead{Start} & \colhead{End} &
\colhead{Conf.} &
\colhead{Calibrator} & \colhead{2nd Calibrator} &
\colhead{Central Freq.}\\
\colhead{}        &
\colhead{[yyyy-mm-dd]}    & \colhead{[hh mm]} & \colhead{[hh mm]} &
\colhead{}           & \colhead{}               &
\colhead{}      & \colhead{[MHz]}
}
\startdata
14B-396	&	2014-09-04	&	11 46	&	13 46	&	D	&	0137+331=3C48	&	J0410+7656	&	1420.208	\\
14B-396	&	2014-11-23	&	08 32	&	10 31	&	C	&	0137+331=3C48	&	J0410+7656	&	1420.208	\\
14B-396	&	2014-11-26	&	08 35	&	10 35	&	C	&	0137+331=3C48	&	J0410+7656	&	1420.208	\\
\enddata
\tablenotetext{a}{VLA Local time in MST/MDT.}
\end{deluxetable*}
